Magnetic Field Energy Harvesting in Railway

Magnetic field energy harvesting (MFEH) is a method by which a system can harness an ambient, alternating magnetic field in order to scavenge energy. Presented in this article is a novel application of the concept aimed at the magnetic fields surrounding the rail current in electrified railway. Due to its non-invasive nature, the approach has the potential to be widely deployed as part of low-cost trackside condition monitoring systems in order to increase lifetime and reduce maintenance requirements. In this work, the viability of MFEH in railway is substantiated experimentally -- two different configurations are assessed both in a controlled laboratory environment, as well as in situ along Norwegian railway. When placed near an emulated section of railway carrying 200 A in the laboratory, the power output of the system is up to 40.5 mW at 50 Hz and 4.15 mW at 16 2/3 Hz. In the field, the prototype system harvests 109 mJ from a single freight train passing by, rendering an estimated daily energy output of 1.14 J in a moderately-trafficked location. It is argued that the approach could indeed eliminate the need for battery replacements, and potentially increase the lifetime of an energy-efficient, battery-powered condition monitoring system indefinitely.

==> bio.tex <==
\begin{IEEEbiography}[{
    \includegraphics[width=1in, height=1.25in, clip, keepaspectratio]
    {aespe_bw.png}
    }]{Asbjørn Engmark Espe}
is a PhD candidate at the Department of Engineering Cybernetics, Norwegian
University of Science and Technology (NTNU). His research interests include
low-power and low-maintenance embedded systems, energy harvesting, and wireless
sensor networks. Espe received his MS degree in cybernetics and robotics from
NTNU in 2019. He is a Member of the IEEE. Contact him at asbjorn.e.espe@ntnu.no.
\end{IEEEbiography}

\begin{IEEEbiography}[{
    \includegraphics[width=1in, height=1.25in, clip, keepaspectratio]
    {thaugan_bw.png}
    }]{Thomas S. Haugan}
is a research scientist at the Department of Electric Power Engineering,
Norwegian University of Science and Technology (NTNU). His research interests
include INTEREST1, INTEREST2, and INTEREST3. Haugan received his MS degree in
FIELD from NTNU in 2012. He is a Member of the IEEE. Contact him at
thomas.s.haugan@ntnu.no.
\end{IEEEbiography}

\begin{IEEEbiography}[{
    \includegraphics[width=1in, height=1.25in, clip, keepaspectratio]
    {gmathisen_bw.png}
    }]{Geir Mathisen}
is a professor at the Department of Engineering Cybernetics, Norwegian
University of Science and Technology (NTNU). His research interests include
INTEREST1, INTEREST2, and INTEREST3. Mathisen received his MS degree in FIELD
from the Norwegian Institute of Technology (NTH) in XXXX, and his Dr.Ing. degree
from NTH in 1996. He is a Senior Member of the IEEE. Contact him at
geir.mathisen@ntnu.no.
\end{IEEEbiography}


==> plot_data_16.tex <==

%%16.67 Hz:
%0.25 m:
\addplot[coil a, model, densely dotted] {0.10338819156701182*x^2};
\addplot[coil a, measured, mark=*]
	coordinates{(25, 58.7) (50, 237.2) (75, 533.8) (100, 974.9) (125, 1512.2) (150, 2234.9) (175, 3098.3) (200, 4151.3)};
\addplot[coil b, model, densely dotted] {0.0663763526819306*x^2};
\addplot[coil b, measured, mark=*]
	coordinates{(25, 48.1) (50, 180.9) (75, 402.8) (100, 743.3) (125, 1162.3) (150, 1743.5) (175, 2406.2) (200, 3228.5)};
%0.5 m:
\addplot[coil a, model, dashed] {0.017314895626866153*x^2};
\addplot[coil a, measured, mark=square*]
	coordinates{(25, 11.2) (50, 41.5) (75, 91.6) (100, 163.1) (125, 250.3) (150, 373.6) (175, 509.4) (200, 680.0)};
\addplot[coil b, model, dashed] {0.011116352857712564*x^2};
\addplot[coil b, measured, mark=square*]
	coordinates{(25, 9.8) (50, 28.8) (75, 62.0) (100, 108.7) (125, 168.5) (150, 244.6) (175, 334.8) (200, 450.1)};
%0.75 m:
\addplot[coil a, model, dashdotted] {0.00488928419540072*x^2};
\addplot[coil a, measured large, mark=triangle*]
	coordinates{(25, 4.3) (50, 12.3) (75, 25.3) (100, 44.5) (125, 67.8) (150, 99.8) (175, 134.3) (200, 179.1)};
\addplot[coil b, model, dashdotted] {0.0031389740665476204*x^2};
\addplot[coil b, measured large, mark=triangle*]
	coordinates{(25, 5.0) (50, 9.3) (75, 18.0) (100, 31.1) (125, 45.9) (150, 64.4) (175, 89.0) (200, 115.3)};
%1.0 m:
\addplot[coil a, model, dashdotdotted] {0.0017819709626767121*x^2};
\addplot[coil a, measured large, mark=diamond*]
	coordinates{(25, 2.9) (50, 6.1) (75, 10.5) (100, 17.3) (125, 25.3) (150, 36.3) (175, 47.6) (200, 64.7)};
\addplot[coil b, model, dashdotdotted] {0.001144044898115123*x^2};
\addplot[coil b, measured large, mark=diamond*]
	coordinates{(25, 4.0) (50, 5.6) (75, 8.9) (100, 13.9) (125, 18.7) (150, 25.4) (175, 32.9) (200, 43.1)};


==> plot_data_50.tex <==

%%50.0 Hz:
%0.25 m:
\addplot[coil a, model, densely dotted] {0.9301216382429436*x^2};
\addplot[coil a, measured, mark=*]
	coordinates{(25, 569.6) (50, 2271.1) (75, 5137.2) (100, 9157.1) (125, 14330.8) (150, 21099.0) (175, 28653.5) (200, 40520.9)};
\addplot[coil b, model, densely dotted] {0.5971482909350695*x^2};
\addplot[coil b, measured, mark=*]
	coordinates{(25, 384.2) (50, 1590.3) (75, 3593.8) (100, 6698.1) (125, 10653.3) (150, 15782.9) (175, 21917.4) (200, 29592.4)};
%0.5 m:
\addplot[coil a, model, dashed] {0.1557717457126405*x^2};
\addplot[coil a, measured, mark=square*]
	coordinates{(25, 101.3) (50, 400.6) (75, 918.6) (100, 1633.1) (125, 2571.1) (150, 3767.6) (175, 5192.0) (200, 6907.6)};
\addplot[coil b, model, dashed] {0.10000716885158564*x^2};
\addplot[coil b, measured, mark=square*]
	coordinates{(25, 61.1) (50, 246.2) (75, 562.6) (100, 1034.5) (125, 1615.3) (150, 2390.9) (175, 3228.5) (200, 4314.1)};
%0.75 m:
\addplot[coil a, model, dashdotted] {0.04398596161452219*x^2};
\addplot[coil a, measured large, mark=triangle*]
	coordinates{(25, 29.3) (50, 114.0) (75, 256.4) (100, 457.4) (125, 712.2) (150, 1040.3) (175, 1427.4) (200, 1889.0)};
\addplot[coil b, model, dashdotted] {0.028239469681477194*x^2};
\addplot[coil b, measured large, mark=triangle*]
	coordinates{(25, 19.3) (50, 67.0) (75, 155.2) (100, 269.6) (125, 434.8) (150, 644.5) (175, 879.8) (200, 1148.1)};
%1.0 m:
\addplot[coil a, model, dashdotdotted] {0.016031325492640327*x^2};
\addplot[coil a, measured large, mark=diamond*]
	coordinates{(25, 11.9) (50, 42.0) (75, 87.2) (100, 161.2) (125, 252.7) (150, 369.2) (175, 502.5) (200, 672.1)};
\addplot[coil b, model, dashdotdotted] {0.010292286756641976*x^2};
\addplot[coil b, measured large, mark=diamond*]
	coordinates{(25, 11.4) (50, 28.8) (75, 58.7) (100, 100.2) (125, 155.2) (150, 220.7) (175, 305.0) (200, 411.2)};

